The Chemical Abundances of Stars in the Halo (CASH) Project. III. A New Classification Scheme for Carbon-Enhanced Metal-poor Stars with S-process Element Enhancement

We present a detailed abundance analysis of 23 elements for a newly discovered carbon-enhanced metal-poor (CEMP) star, HE 0414-0343, from the Chemical Abundances of Stars in the Halo (CASH) Project. Its spectroscopic stellar parameters are Teff = 4863 K, log g = 1.25, vmic = 2.20 km/s, and [Fe/H] = -2.24. Radial velocity measurements covering seven years indicate HE 0414-0343 to be a binary. HE 0414-0343 has [C/Fe] = 1.44 and is strongly enhanced in neutron-capture elements but its abundances cannot be reproduced by a solar-type s-process pattern alone. Traditionally, it could be classified as "CEMP-r/s" star. Based on abundance comparisons with AGB star nucleosynthesis models, we suggest a new physically-motivated origin and classification scheme for CEMP-s stars and the still poorly-understood CEMP-r/s. The new scheme describes a continuous transition between these two so-far distinctly treated subgroups: CEMP-sA, CEMP-sB, and CEMP-sC. Possible causes for a continuous transition include the number of thermal pulses the AGB companion underwent, the effect of different AGB star masses on their nucleosynthetic yields, and physics that is not well approximated in 1-D stellar models such as proton ingestion episodes and rotation. Based on a set of detailed AGB models, we suggest the abundance signature of HE 0414-0343 to have arisen from a >1.3 Msun mass AGB star and a late-time mass transfer, that transformed HE 0414-0343 into a CEMP-sC star. We also find the [Y/Ba] ratio well parametrizes the classification and can thus be used to easily classify any future such stars.

==> eqwtabnew.tex <==
\begin{deluxetable}{lccrrr}
  \tablecolumns{6} 
  \tablewidth{0pc} 
  \tablecaption{Equivalent Widths and Abundances}
  \tablehead{\colhead{Species}&\colhead{$\lambda$}& \colhead{$\chi$} &\colhead{log gf}& \colhead{W} &\colhead{$\log\epsilon$(X)}\\ 
 \colhead{}&\colhead{[\AA{}]}& \colhead{[eV]}&\colhead{} &\colhead{m\AA{}} &\colhead{}}
\startdata
C$_{2}$  & 5165     & \nodata &  \nodata & Synth & 7.63   \\
C$^{12}$/C$^{13}$& \nodata  & \nodata &  \nodata & Synth & 5\tablenotemark{a}      \\
Mg I &  4571.09  &  0.00  &  $-$5.69  &  98.7  &  5.94 \\
Mg I &  4702.99  &  4.33  &  $-$0.38  &  111.1  &  5.81 \\
Mg I &  5172.68  &  2.71  &  $-$0.45  &  240.5  &  5.75 \\
Mg I &  5528.40  &  4.34  &  $-$0.50  &  107.2  &  5.84 \\
Mg I &  5711.09  &  4.34  &  $-$1.72  &  24.7  &  5.76 \\
Ca I &  4455.89  &  1.90  &  $-$0.53  &  88.6  &  4.76 \\
Ca I &  5581.97  &  2.52  &  $-$0.56  &  34.0  &  4.51 \\
Ca I &  5588.76  &  2.52  &     0.21  &  80.2  &  4.49 \\
Ca I &  5590.12  &  2.52  &  $-$0.57  &  25.5  &  4.35 \\
Ca I &  5594.46  &  2.52  &     0.10  &  85.8  &  4.70 \\
Ca I &  5598.48  &  2.52  &  $-$0.09  &  68.6  &  4.60 \\
Ca I &  5601.28  &  2.53  &  $-$0.52  &  40.4  &  4.60 \\
Ca I &  5857.45  &  2.93  &     0.23  &  55.7  &  4.54 \\
Ca I &  6102.72  &  1.88  &  $-$0.79  &  63.5  &  4.46 \\
Ca I &  6122.22  &  1.89  &  $-$0.32  &  97.4  &  4.53 \\
Ca I &  6162.17  &  1.90  &  $-$0.09  &  102.1  &  4.39 \\
Ca I &  6439.07  &  2.52  &     0.47  &  102.0  &  4.55 \\
Ca I &  6449.81  &  2.52  &  $-$0.50  &  54.4  &  4.76 \\
Ca I &  6499.64  &  2.52  &  $-$0.82  &  35.2  &  4.76 \\
Sc II&  4415.54  &  0.59  &  $-$0.67  &  109.5  &  1.14 \\
Sc II&  5031.01  &  1.36  &  $-$0.40  &  71.9  &  1.02 \\
Sc II&  5031.01  &  1.36  &  $-$0.40  &  79.9  &  1.14 \\
Sc II&  5239.81  &  1.46  &  $-$0.77  &  68.0  &  1.43 \\
Sc II&  5526.78  &  1.77  &     0.02  &  70.0  &  1.01 \\
Sc II&  5641.00  &  1.50  &  $-$1.13  &  24.7  &  1.11 \\
Sc II&  5657.90  &  1.51  &  $-$0.60  &  51.2  &  1.04 \\
Sc II&  5658.36  &  1.50  &  $-$1.21  &  24.2  &  1.18 \\
Sc II&  5667.16  &  1.50  &  $-$1.31  &  28.5  &  1.37 \\
Sc II&  5684.21  &  1.51  &  $-$1.07  &  18.2  &  0.90 \\
Ti I &  3998.64  &  0.05  &     0.01  &  83.3  &  2.63 \\
Ti I &  4518.02  &  0.83  &  $-$0.27  &  42.6  &  3.06 \\
Ti I &  4533.24  &  0.85  &     0.53  &  67.0  &  2.66 \\
Ti I &  4534.78  &  0.84  &     0.34  &  58.0  &  2.70 \\
Ti I &  4535.56  &  0.83  &     0.12  &  55.8  &  2.87 \\
Ti I &  4548.76  &  0.83  &  $-$0.30  &  35.1  &  2.95 \\
Ti I &  4555.49  &  0.85  &  $-$0.43  &  35.2  &  3.11 \\
Ti I &  4656.47  &  0.00  &  $-$1.29  &  31.9  &  2.91 \\
Ti I &  4681.91  &  0.05  &  $-$1.01  &  63.8  &  3.20 \\
Ti I &  4840.87  &  0.90  &  $-$0.45  &  22.5  &  2.91 \\
Ti I &  4840.87  &  0.90  &  $-$0.45  &  25.1  &  2.97 \\
Ti I &  4981.73  &  0.84  &  0.56  &  85.7  &  2.88 \\
Ti I &  4981.73  &  0.84  &  0.56  &  90.8  &  2.98 \\
Ti I &  4991.07  &  0.84  &  0.44  &  87.1  &  3.02 \\
Ti I &  4991.07  &  0.84  &  0.44  &  96.5  &  3.20 \\
Ti I &  5007.20  &  0.82  &  0.17  &  85.6  &  3.25 \\
Ti I &  5007.20  &  0.82  &  0.17  &  88.2  &  3.29 \\
Ti I &  5016.16  &  0.85  &  $-$0.52  &  26.8  &  3.00 \\
Ti I &  5016.16  &  0.85  &  $-$0.52  &  28.5  &  3.04 \\
Ti I &  5020.02  &  0.84  &  $-$0.36  &  28.0  &  2.86 \\
Ti I &  5024.84  &  0.82  &  $-$0.55  &  26.8  &  3.00 \\
Ti I &  5024.84  &  0.82  &  $-$0.55  &  28.8  &  3.04 \\
Ti I &  5035.90  &  1.46  &  0.26  &  28.1  &  2.95 \\
Ti I &  5035.90  &  1.46  &  0.26  &  35.9  &  3.10 \\
Ti I &  5036.46  &  1.44  &  0.19  &  19.0  &  2.79 \\
Ti I &  5036.46  &  1.44  &  0.19  &  23.5  &  2.90 \\
Ti I &  5039.96  &  0.02  &  $-$1.13  &  55.6  &  3.12 \\
Ti I &  5039.96  &  0.02  &  $-$1.13  &  57.3  &  3.15 \\
Ti I &  5064.65  &  0.05  &  $-$0.94  &  71.1  &  3.20 \\
Ti I &  5210.39  &  0.05  &  $-$0.83  &  65.3  &  2.99 \\
Ti II&  4418.33  &  1.24  &  $-$1.97  &  84.1  &  3.12 \\
Ti II&  4441.73  &  1.18  &  $-$2.41  &  85.3  &  3.51 \\
Ti II&  4464.44  &  1.16  &  $-$1.81  &  97.1  &  3.10 \\
Ti II&  4470.85  &  1.17  &  $-$2.02  &  105.6  &  3.49 \\
Ti II&  4488.34  &  3.12  &  $-$0.82  &  21.2  &  3.03 \\
Ti II&  4529.48  &  1.57  &  $-$2.03  &  77.7  &  3.43 \\
Ti II&  4563.77  &  1.22  &  $-$0.96  &  138.8  &  3.17 \\
Ti II&  4583.40  &  1.16  &  $-$2.92  &  27.2  &  3.01 \\
Ti II&  4589.91  &  1.24  &  $-$1.79  &  90.0  &  3.01 \\
Ti II&  4636.32  &  1.16  &  $-$3.02  &  29.5  &  3.16 \\
Ti II&  4657.20  &  1.24  &  $-$2.24  &  58.6  &  2.94 \\
Ti II&  4708.66  &  1.24  &  $-$2.34  &  67.8  &  3.17 \\
Ti II&  4779.97  &  2.05  &  $-$1.37  &  62.7  &  3.07 \\
Ti II&  4798.53  &  1.08  &  $-$2.68  &  61.0  &  3.21 \\
Ti II&  4805.08  &  2.06  &  $-$1.10  &  84.7  &  3.17 \\
Ti II&  4805.08  &  2.06  &  $-$1.10  &  89.8  &  3.25 \\
Ti II&  4865.61  &  1.12  &  $-$2.81  &  29.8  &  2.89 \\
Ti II&  4865.61  &  1.12  &  $-$2.81  &  45.7  &  3.15 \\
Ti II&  4911.17  &  3.12  &  $-$0.34  &  43.8  &  2.97 \\
Ti II&  5185.90  &  1.89  &  $-$1.49  &  62.7  &  2.97 \\
Ti II&  5226.53  &  1.57  &  $-$1.26  &  124.2  &  3.41 \\
Ti II&  5336.78  &  1.58  &  $-$1.59  &  96.0  &  3.21 \\
Ti II&  5381.02  &  1.57  &  $-$1.92  &  64.3  &  3.03 \\
Ti II&  5418.76  &  1.58  &  $-$2.00  &  46.7  &  2.86 \\
Cr I &  4545.95  &  0.94  &  $-$1.37  &  31.4  &  3.27 \\
Cr I &  4600.75  &  1.00  &  $-$1.26  &  40.1  &  3.38 \\
Cr I &  4626.18  &  0.97  &  $-$1.32  &  32.6  &  3.27 \\
Cr I &  4646.15  &  1.03  &  $-$0.74  &  69.1  &  3.36 \\
Cr I &  4652.15  &  1.00  &  $-$1.03  &  48.3  &  3.28 \\
Cr I &  5206.04  &  0.94  &     0.02  & 113.1  &  3.24 \\
Cr I &  5247.56  &  0.96  &  $-$1.64  &  18.8  &  3.24 \\
Cr I &  5296.69  &  0.98  &  $-$1.36  &  27.5  &  3.18 \\
Cr I &  5348.31  &  1.00  &  $-$1.21  &  35.9  &  3.21 \\
Cr I &  5409.77  &  1.03  &  $-$0.67  &  68.9  &  3.22 \\
Mn I &  4754.04  &  2.28  &  $-$0.09  & Synth  &  2.71 \\
Mn I &  4783.52  &  2.32  &     0.14  & Synth  &  2.79 \\
Fe I &  4443.19  &  2.86  &  $-$1.04  &  71.1  &  5.32 \\
Fe I &  4466.55  &  2.83  &  $-$0.60  &  99.2  &  5.40 \\
Fe I &  4476.01  &  2.85  &  $-$0.82  &  88.6  &  5.42 \\
Fe I &  4484.22  &  3.60  &  $-$0.86  &  36.1  &  5.40 \\
Fe I &  4592.65  &  1.56  &  $-$2.46  &  79.8  &  5.37 \\
Fe I &  4632.91  &  1.61  &  $-$2.91  &  51.8  &  5.41 \\
Fe I &  4643.46  &  3.64  &  $-$1.15  &  21.1  &  5.41 \\
Fe I &  4678.84  &  3.60  &  $-$0.83  &  39.3  &  5.41 \\
Fe I &  4859.74  &  2.88  &  $-$0.76  &  92.7  &  5.41 \\
Fe I &  4859.74  &  2.88  &  $-$0.76  &  92.7  &  5.41 \\
Fe I &  4903.31  &  2.88  &  $-$0.93  &  60.4  &  5.01 \\
Fe I &  4903.31  &  2.88  &  $-$0.93  &  67.9  &  5.13 \\
Fe I &  4918.99  &  2.85  &  $-$0.34  &  99.3  &  5.08 \\
Fe I &  4918.99  &  2.85  &  $-$0.34  &  99.3  &  5.08 \\
Fe I &  4924.77  &  2.28  &  $-$2.11  &  39.9  &  5.17 \\
Fe I &  4924.77  &  2.28  &  $-$2.11  &  47.1  &  5.29 \\
Fe I &  4938.81  &  2.88  &  $-$1.08  &  58.5  &  5.13 \\
Fe I &  4938.81  &  2.88  &  $-$1.08  &  63.6  &  5.21 \\
Fe I &  4966.08  &  3.33  &  $-$0.87  &  41.0  &  5.15 \\
Fe I &  4966.08  &  3.33  &  $-$0.87  &  46.7  &  5.25 \\
Fe I &  4973.10  &  3.96  &  $-$0.95  &  17.6  &  5.45 \\
Fe I &  4994.13  &  0.92  &  $-$2.97  &  97.9  &  5.39 \\
Fe I &  4994.13  &  0.92  &  $-$2.97  &  98.8  &  5.42 \\
Fe I &  5006.11  &  2.83  &  $-$0.61  &  87.1  &  5.07 \\
Fe I &  5006.11  &  2.83  &  $-$0.61  &  88.7  &  5.11 \\
Fe I &  5014.94  &  3.94  &  $-$0.30  &  44.1  &  5.33 \\
Fe I &  5014.94  &  3.94  &  $-$0.30  &  44.9  &  5.34 \\
Fe I &  5041.07  &  0.96  &  $-$3.09  &  96.9  &  5.54 \\
Fe I &  5041.75  &  1.49  &  $-$2.20  &  98.4  &  5.30 \\
Fe I &  5049.82  &  2.28  &  $-$1.35  &  89.4  &  5.22 \\
Fe I &  5049.82  &  2.28  &  $-$1.35  &  93.6  &  5.30 \\
Fe I &  5051.63  &  0.92  &  $-$2.76  &  99.8  &  5.21 \\
Fe I &  5051.63  &  0.92  &  $-$2.76  &  99.8  &  5.21 \\
Fe I &  5068.76  &  2.94  &  $-$1.04  &  77.0  &  5.45 \\
Fe I &  5074.74  &  4.22  &  $-$0.20  &  35.2  &  5.39 \\
Fe I &  5079.22  &  2.20  &  $-$2.10  &  52.2  &  5.25 \\
Fe I &  5127.36  &  0.92  &  $-$3.25  &  83.4  &  5.39 \\
Fe I &  5141.73  &  2.42  &  $-$2.24  &  30.2  &  5.27 \\
Fe I &  5142.92  &  0.96  &  $-$3.08  &  99.2  &  5.55 \\
Fe I &  5192.34  &  3.00  &  $-$0.42  &  95.5  &  5.22 \\
Fe I &  5198.71  &  2.22  &  $-$2.09  &  50.8  &  5.24 \\
Fe I &  5202.33  &  2.18  &  $-$1.87  &  72.5  &  5.31 \\
Fe I &  5216.27  &  1.61  &  $-$2.08  &  85.9  &  5.07 \\
Fe I &  5217.39  &  3.21  &  $-$1.16  &  37.0  &  5.22 \\
Fe I &  5242.49  &  3.63  &  $-$0.97  &  20.4  &  5.17 \\
Fe I &  5263.30  &  3.27  &  $-$0.88  &  49.4  &  5.21 \\
Fe I &  5266.55  &  3.00  &  $-$0.39  &  87.5  &  5.04 \\
Fe I &  5281.79  &  3.04  &  $-$0.83  &  62.6  &  5.11 \\
Fe I &  5283.62  &  3.24  &  $-$0.52  &  77.3  &  5.27 \\
Fe I &  5302.30  &  3.28  &  $-$0.72  &  64.1  &  5.30 \\
Fe I &  5307.36  &  1.61  &  $-$2.91  &  46.1  &  5.26 \\
Fe I &  5324.17  &  3.21  &  $-$0.10  &  93.5  &  5.09 \\
Fe I &  5332.90  &  1.55  &  $-$2.78  &  56.4  &  5.22 \\
Fe I &  5339.93  &  3.27  &  $-$0.72  &  59.0  &  5.20 \\
Fe I &  5364.87  &  4.45  &     0.23  &  34.6  &  5.20 \\
Fe I &  5365.40  &  3.56  &  $-$1.02  &  19.7  &  5.11 \\
Fe I &  5367.46  &  4.42  &     0.44  &  39.2  &  5.04 \\
Fe I &  5369.96  &  4.37  &     0.54  &  53.0  &  5.11 \\
Fe I &  5389.47  &  4.42  &  $-$0.41  &  13.1  &  5.27 \\
Fe I &  5410.91  &  4.47  &     0.40  &  36.5  &  5.08 \\
Fe I &  5415.19  &  4.39  &     0.64  &  52.6  &  5.02 \\
Fe I &  5424.06  &  4.32  &     0.52  &  74.7  &  5.43 \\
Fe I &  5569.61  &  3.42  &  $-$0.54  &  66.3  &  5.29 \\
Fe I &  5572.84  &  3.40  &  $-$0.28  &  71.7  &  5.10 \\
Fe I &  5576.08  &  3.43  &  $-$1.00  &  44.6  &  5.43 \\
Fe I &  5586.75  &  3.37  &  $-$0.14  &  78.4  &  5.03 \\
Fe I &  5615.64  &  3.33  &     0.05  &  98.5  &  5.15 \\
Fe I &  5624.54  &  3.42  &  $-$0.76  &  51.4  &  5.28 \\
Fe I &  5658.81  &  3.40  &  $-$0.79  &  46.7  &  5.21 \\
Fe I &  5662.51  &  4.18  &  $-$0.57  &  15.4  &  5.23 \\
Fe I &  5701.54  &  2.56  &  $-$2.14  &  26.1  &  5.22 \\
Fe I &  6065.48  &  2.61  &  $-$1.41  &  71.0  &  5.26 \\
Fe I &  6136.61  &  2.45  &  $-$1.41  &  82.8  &  5.26 \\
Fe I &  6137.69  &  2.59  &  $-$1.35  &  74.8  &  5.24 \\
Fe I &  6191.55  &  2.43  &  $-$1.42  &  84.4  &  5.27 \\
Fe I &  6200.31  &  2.61  &  $-$2.44  &  20.2  &  5.41 \\
Fe I &  6213.42  &  2.22  &  $-$2.48  &  44.6  &  5.46 \\
Fe I &  6230.72  &  2.56  &  $-$1.28  &  84.0  &  5.28 \\
Fe I &  6252.55  &  2.40  &  $-$1.69  &  68.5  &  5.25 \\
Fe I &  6254.25  &  2.28  &  $-$2.44  &  47.3  &  5.53 \\
Fe I &  6322.68  &  2.59  &  $-$2.47  &  20.7  &  5.43 \\
Fe I &  6335.33  &  2.20  &  $-$2.18  &  48.1  &  5.19 \\
Fe I &  6393.60  &  2.43  &  $-$1.58  &  84.4  &  5.42 \\
Fe I &  6400.00  &  3.60  &  $-$0.29  &  65.5  &  5.20 \\
Fe I &  6411.64  &  3.65  &  $-$0.59  &  47.9  &  5.28 \\
Fe I &  6421.35  &  2.28  &  $-$2.01  &  64.1  &  5.35 \\
Fe I &  6430.84  &  2.18  &  $-$1.95  &  87.8  &  5.54 \\
Fe I &  6592.91  &  2.73  &  $-$1.47  &  52.2  &  5.15 \\
Fe II&  4489.18  &  2.83  &  $-$2.97  &  47.7  &  5.28 \\
Fe II&  4508.28  &  2.86  &  $-$2.58  &  68.5  &  5.26 \\
Fe II&  4515.34  &  2.84  &  $-$2.60  &  75.8  &  5.38 \\
Fe II&  4520.22  &  2.81  &  $-$2.60  &  64.1  &  5.15 \\
Fe II&  4583.84  &  2.81  &  $-$1.93  &  95.3  &  5.05 \\
Fe II&  4620.52  &  2.83  &  $-$3.21  &  36.3  &  5.32 \\
Fe II&  4731.43  &  2.89  &  $-$3.36  &  29.4  &  5.40 \\
Fe II&  4993.35  &  2.81  &  $-$3.67  &  13.6  &  5.19 \\
Fe II&  4993.35  &  2.81  &  $-$3.67  &  17.9  &  5.33 \\
Fe II&  5197.58  &  3.23  &  $-$2.22  &  62.7  &  5.18 \\
Fe II&  5234.63  &  3.22  &  $-$2.18  &  61.9  &  5.11 \\
Fe II&  5276.00  &  3.20  &  $-$2.01  &  70.7  &  5.06 \\
Fe II&  5284.08  &  2.89  &  $-$3.19  &  30.2  &  5.21 \\
Fe II&  5325.55  &  3.22  &  $-$3.16  &  16.1  &  5.22 \\
Fe II&  5534.83  &  3.25  &  $-$2.93  &  27.1  &  5.29 \\
Fe II&  6247.54  &  3.89  &  $-$2.51  &  20.5  &  5.42 \\
Fe II&  6432.68  &  2.89  &  $-$3.71  &  22.2  &  5.51 \\
Fe II&  6456.38  &  3.90  &  $-$2.08  &  37.2  &  5.34 \\
Ni I &  4605.00  &  3.48  &  $-$0.29  &  22.5  &  4.10 \\
Ni I &  4648.65  &  3.42  &  $-$0.16  &  23.7  &  3.92 \\
Ni I &  4855.41  &  3.54  &  0.00  &  20.7  &  3.81 \\
Ni I &  4904.41  &  3.54  &  $-$0.17  &  12.2  &  3.71 \\
Ni I &  4904.41  &  3.54  &  $-$0.17  &  20.3  &  3.97 \\
Ni I &  4980.16  &  3.61  &  $-$0.11  &  22.6  &  4.05 \\
Ni I &  4980.16  &  3.61  &  $-$0.11  &  25.0  &  4.10 \\
Ni I &  5035.37  &  3.63  &  0.29  &  22.7  &  3.67 \\
Ni I &  5035.37  &  3.63  &  0.29  &  34.7  &  3.92 \\
Ni I &  5080.52  &  3.65  &  0.13  &  34.2  &  4.09 \\
Ni I &  5081.11  &  3.85  &  0.30  &  15.6  &  3.71 \\
Ni I &  5084.08  &  3.68  &  0.03  &  16.1  &  3.80 \\
Ni I &  5754.67  &  1.94  &  $-$2.33  &  25.2  &  4.37 \\
Ni I &  6643.64  &  1.68  &  $-$2.30  &  33.4  &  4.14 \\
Ni I &  6767.77  &  1.83  &  $-$2.17  &  34.6  &  4.20 \\
Zn I  & 4810.52  &  4.08  &  $-$0.13  & Synth  &  2.38 \\
Sr II   & 3464.45  &   3.04  &    0.49  & Synth &  1.11   \\
Y II    & 4883.68  &   1.08  &    0.07  & Synth & 0.13 \\
Y II    & 5087.42  &   1.08  & $-$0.17  & Synth & 0.21 \\
Zr II & 4208.99 & 0.71 &$-$0.46 & Synth & 0.71 \\
Zr II & 4613.95 & 0.97 &$-$1.54 & Synth & 0.87 \\
Zr II & 5112.28 & 1.66 &$-$0.59 & Synth & 0.99 \\
Ba II & 5853.69 & 0.60 &$-$0.91 & Synth & 1.80 \\
Ba II & 6141.73 & 0.70 &$-$0.08 & Synth & 1.77 \\
Ba II & 6496.91 & 0.60 &$-$0.38 & Synth & 1.87 \\
La II & 4740.28 & 0.13 &$-$0.94 & Synth & 0.45 \\
La II & 4748.73 & 0.93 &$-$0.54 & Synth & 0.42 \\
La II & 4824.05 & 0.65 &$-$1.19 & Synth & 0.64 \\
La II & 6262.29 & 0.40 &$-$1.24 & Synth & 0.40 \\
La II & 6390.48 & 0.32 &$-$1.45 & Synth & 0.41 \\
Ce II & 4739.51 & 1.25 &$-$0.53 & Synth & 0.67 \\
Ce II & 4739.52 & 0.53 &$-$1.02 & Synth & 0.69 \\
Ce II & 4747.26 & 0.90 &$-$1.79 & Synth & 0.89 \\
Ce II & 4882.46 & 1.53 &0.19 & Synth & 0.70 \\
Pr II & 4744.91 & 0.20 &$-$1.14 & Synth & $-$0.17 \\
Nd II & 5310.04 & 1.14 &$-$0.98 & Synth & 0.83 \\
Nd II & 5311.45 & 0.98 &$-$0.42 & Synth & 0.87 \\
Nd II & 5319.81 & 0.55 &$-$0.14 & Synth & 0.73 \\
Sm II & 4318.93 & 0.28 &$-$0.25 & Synth & 0.04 \\
Sm II & 4434.32 & 0.38 &$-$0.07 & Synth & 0.17 \\
Sm II & 4519.63 & 0.54 &$-$0.35 & Synth & 0.21 \\
Eu II & 6645.06 & 1.38 &0.20 & Synth & $-$0.49 \\
Dy II & 4449.70 & 0.00 &$-$1.03 & Synth & 0.45 \\
Er I & 3682.70 & 0.89 &$-$0.38 & Synth & 0.24 \\
Yb II & 3694.19 & 0.00 &$-$0.82 & Synth & 0.03 \\
Pb I & 3683.46 & 0.97 &$-$0.46 & Synth & 1.97 \\
Pb I & 4057.81 & 1.32 &$-$0.22 & Synth & 2.11 \\
\enddata
\tablenotetext{a}{The C$^{12}$/C$^{13}$ value is a ratio and not a $\log\epsilon$(X) value.}
\label{synthtab}
\end{deluxetable} 

